A Probabilistic Approach to Learning the Degree of Equivariance in Steerable CNNs

Steerable convolutional neural networks (SCNNs) enhance task performance by modelling geometric symmetries through equivariance constraints on weights. Yet, unknown or varying symmetries can lead to overconstrained weights and decreased performance. To address this, this paper introduces a probabilistic method to learn the degree of equivariance in SCNNs. We parameterise the degree of equivariance as a likelihood distribution over the transformation group using Fourier coefficients, offering the option to model layer-wise and shared equivariance. These likelihood distributions are regularised to ensure an interpretable degree of equivariance across the network. Advantages include the applicability to many types of equivariant networks through the flexible framework of SCNNs and the ability to learn equivariance with respect to any subgroup of any compact group without requiring additional layers. Our experiments reveal competitive performance on datasets with mixed symmetries, with learnt likelihood distributions that are representative of the underlying degree of equivariance.

==> TodoChanges.tex <==


- include theoretical and experimental DONE comparison to wang
- DONE reviewer 1 point 4: Mention in future work that we do not have theoretical proof that the learnt equivariance matches true equivariance and leave this as future work
- DONE reviewer 1 point 6: Mention in the normalization that other normalisations can also work, but that Softmax provides an advantage for KL. Mention the example of Parseval identity in footnote
- DONE Clarify notation of [0(ii)] and [j'(Jl)] on line 155
- DONE With "interpretable", we indeed mean that the degree of equivariance can directly be interpreted from the learnt distribution. We will make it more explicit.
- DONE Include a limitation section

- Improve flow of equations in equations 4, 5, 6 and supp C.2 Solving Equivariance Constraints
- DONE Expand section 3.4 with a deeper computational analysis.
    - Re-write 3.4 to rephrase why our implementation might be suboptimal (caching and steerable basis). Point to this discussion in limitations
- Done Clarify the effect of the learnt likelihood on the model's equivariance a bit more explicitly.
- DONE Mention explicitly that Double MNIST includes data augmentation during training.
- Yes do! Mention for future work a comparison with or inclusion within ViTs

- DONEInclude number of parameters for our models and baselines
    - run RPP on jetflow, include params, include RPP performance with star and explain that it is our run and we do not know the config. Refer here and in bandlimniting section to Apx for more in-depth parameter count
- DONEInclude limitations section

- DONE Discuss monotonically decreasing equivariance vs not (contradictory with Romero). Mention quickly that we observed this to be better in our experiments, but did not do a lot of research. More for future work. Do this in appendix and point to it in KL divergence section
- DONE Discuss sparse alignment loss being sufficient for our experiments, potentially due to low bandlimiting
-DONE Use param counts to convey that band-limiting is not necessary, but a tool In appendix
DONE - Clarify that we use the Haar measure.


Finish writing F.2 (model architectures) and DONE F.1.4.

DONE? Finish writing appendix discussing monotonically decreasing equivariance

DONE add image in front page

DONE Finish writing monotonically appendix


--!!! Mention detaching previous layer for KL. Possibly in main paper, otherwise in D.2. In D.2. mention that they do not detach layer n

-- DONE cite jetflow and smoke from phiflow and nasa

-- DONE change f.2 last paragraph. Mention that we sanity checked by re-running and achieved similar perf

-- DONE Make G.5 table 23 more clear that 5x5 is hypothetical by separating it from the rest. 

-- Try to add RPP numbers on Smoke G.5 table 23

-- DONE check loss function for F.4. table 14 smoke and jetflow

-- DONE reference the repo

-- DONE add color to equations (e.g. Y in eq 5, j and k in indices) and own color for lambda

